PromptHSI: Universal Hyperspectral Image Restoration with Vision-Language Modulated Frequency Adaptation

Recent advances in All-in-One (AiO) RGB image restoration have demonstrated the effectiveness of prompt learning in handling multiple degradations within a single model. However, extending these approaches to hyperspectral image (HSI) restoration is challenging due to the domain gap between RGB and HSI features, information loss in visual prompts under severe composite degradations, and difficulties in capturing HSI-specific degradation patterns via text prompts. In this paper, we propose PromptHSI, the first universal AiO HSI restoration framework that addresses these challenges. By incorporating frequency-aware feature modulation, which utilizes frequency analysis to narrow down the restoration search space and employing vision-language model (VLM)-guided prompt learning, our approach decomposes text prompts into intensity and bias controllers that effectively guide the restoration process while mitigating domain discrepancies. Extensive experiments demonstrate that our unified architecture excels at both fine-grained recovery and global information restoration across diverse degradation scenarios, highlighting its significant potential for practical remote sensing applications. The source code is available at https://github.com/chingheng0808/PromptHSI.

==> supplementary_arxiv.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \usepackage{cvpr}
% \usepackage{pifont}
% %--------------------------
% \usepackage{mathtools}
% \usepackage{balance}
% %--------------------------
% %---------
% \usepackage{xcolor}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage{graphics}
% \usepackage{float}
% \usepackage{calc}
% \usepackage{amsfonts,bm,url,color,theorem}
% \usepackage{psfrag}
% \usepackage{multirow,epsfig}
% \usepackage{diagbox} 
% \usepackage{hhline}
% \usepackage{caption}
% \usepackage{adjustbox}
% \usepackage{makecell}
% \usepackage{etex}
% %\usepackage{newclude}
% \usepackage{placeins}
% \usepackage[dvipsnames]{xcolor}
% \usepackage{tcolorbox}
% %--------------------------
% \usepackage{mathtools}
% \DeclarePairedDelimiter\ceil{\lceil}{\rceil}
% \DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
% %--------------------------
% \def\blue{\color{blue}}
% \def\red{\color{red}}
% %---------

% \usepackage[table,xcdraw]{xcolor}
% \usepackage{colortbl} 

% % 定義顏色
% \definecolor{bestColor}{RGB}{255, 0, 0}    % 最佳 - 紅色
% \definecolor{secondBestColor}{RGB}{0, 0, 255} % 次佳 - 藍色
% \definecolor{thirdBestColor}{RGB}{0, 100, 0}  % 第三佳 - 深綠色

% \definecolor{cnn_color}{RGB}{240,248,255}  % Alice Blue
% \definecolor{transformer_color}{RGB}{255,250,240}  % Floral White
% \definecolor{ours_color}{RGB}{245,255,250}  % Mint Cream

% % 定義簡易指令
% \newcommand{\best}[1]{\textcolor{bestColor}{\textbf{#1}}}      % 最佳
% \newcommand{\secondBest}[1]{\textcolor{secondBestColor}{\textbf{#1}}} % 次佳
% \newcommand{\thirdBest}[1]{\textcolor{thirdBestColor}{\textbf{#1}}}  % 第三佳

% %========================================================================================
% %make sure to keep this for convenience later



% %========================================================================================

% \definecolor{background_color}{RGB}{255,255,255}  % Alice Blue

% \definecolor{cnn_color}{RGB}{240,248,255}  % Alice Blue
% \definecolor{transformer_color}{RGB}{255,250,240}  % Floral White
% \definecolor{ours_color}{RGB}{240,255,240}  % Mint Cream
% \definecolor{input_color}{RGB}{255,240,240}      % 淺灰色


% % Define the colors
% \definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
% \definecolor{best}{rgb}{1,0,0}      % Red
% \definecolor{secondbest}{rgb}{0,0,1}

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \usepackage[pagebackref,breaklinks,colorlinks,allcolors=cvprblue]{hyperref}

% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}


% \begin{document}

% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{PromptHSI: Universal Hyperspectral Image Restoration Framework for Composite Degradation}  % **** Enter the paper title here
% \author{Supplementary Material}


% \thispagestyle{empty}
\twocolumn[{%
   \renewcommand\twocolumn[1][]{#1}%
   \maketitle
   \vspace{-6mm} 
   \begin{center}
       {\LARGE \textbf{Supplementary Materials}}
       \vspace{16mm} % 增加标题与图片的间距
       
       \centering
       \includegraphics[width=\linewidth]{figures/tsne_compare_compressed.pdf}
       
       \vspace{-2mm} % 调整 caption 与图片的距离
       \captionof{figure}{\small \underline{\textbf{The t-SNE map visualization for the proposed PromptHSI and other All-in-One RGR image restoration methods.}} Note that for training PromptHSI, the generated dataset includes various degradations, with each type presented separately instead of concurrently. Subsequently, we visualize the t-SNE map with \ding{182} \textbf{\emph{Top:}} multiple degradation; \ding{183} \textbf{\emph{Bottom:}} composite degradation during testing-time.}
       \label{fig:teaser}
       
       \vspace{6mm} % 调整图片与正文之间的间距
   \end{center}%
}]

\appendix

%%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW

%-------------------------------------------------------------------------
% 挑幾個好的範例說明controllable


\input{sections/overview_sup}

\input{sections/dataset_sup}

\input{sections/architecture_sup}

\input{sections/experiments_sup}


% \clearpage
% \clearpage
% \balance

%%%%%%%%% REFERENCES
% \section*{References}
% \bibliographystyle{ieee_fullname} 
% \bibliography{egbib}
% \begingroup
% \footnotesize
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% \endgroup


% \end{document}


==> tables/004_demo.tex <==
\begin{table*}[t]
\parbox{.32\linewidth}{
\centering
\caption{\small Ablation of integration strategy. } 
\label{table:ablation_condition_information}
\vspace{-3mm}
\setlength{\tabcolsep}{2pt}
\scalebox{0.69}{
\begin{tabular}{c | c }
\toprule[0.15em]
Sampling Order & PSNR / SAM / RMSE / EGRAS \\
\hline
Only Intensity & \secondBest{28.786} / 2.894 / 0.0184 / 5.091 \\
Only Bias & 28.773 / 2.868 / 0.0157 / \secondBest{5.043} \\
CLIP-adapter & 28.761 / \secondBest{2.867} / \best{0.0150} / 5.239 \\ \hline
\textbf{Intensity \& Bias}& \best{28.788} / \best{2.852} / \secondBest{0.0151} / \best{5.039} \\
%
\bottomrule[0.15em]
\end{tabular}}}
\hfill
\parbox{.31\linewidth}{
\centering
\caption{\small Ablation of loss function. }
\label{table:ablation_loss}
\vspace{-3mm}
\setlength{\tabcolsep}{2pt}
\scalebox{0.68}{
\begin{tabular}{cccc|c}
\toprule[0.15em]
$\ell_1$&$\ell_\text{SAM}$&$\ell_\text{SWT}$& $\ell_\text{BMSE}$& PSNR / SAM / RMSE / EGRAS \\ 
\hline
%
	$\surd$& & & & \best{28.937} / 3.096 / \best{0.0147} / 5.103\\
	$\surd$&$\surd$& & & 28.649 / \secondBest{2.869} / 0.0154 / \secondBest{5.074}\\
	$\surd$&$\surd$&$\surd$& & 28.701 / 2.878 / 0.0152 / 5.110 \\ \hline
	$\surd$&$\surd$&$\surd$&$\surd$& \secondBest{28.788} / \best{2.852} / \secondBest{0.0151} / \best{5.039} \\
%
\bottomrule[0.15em]
\end{tabular}
}}
\hfill
\parbox{.36\linewidth}{
\centering
\caption{\small Ablation of length of text prompt. }
\label{table:ablation_ref}
\vspace{-3mm}
\setlength{\tabcolsep}{4pt}
\scalebox{0.69}{
\begin{tabular}{c|c|c|c}
\toprule[0.15em]
$\text{Spe}$, $\text{Spa}$, $\text{Rec}$ &\text{PSNR} / \text{SAM} / \text{RMSE} / \text{EGRAS} &FLOPs&Params \\
\hline
%
4, 4, 1 & 39.251 / 1.254 / 23.514 / 1.453 & 385G &  12.7M \\ 
4, 4, 2 & 40.869 / 1.197 / 21.283 / 1.387 & 554G & 15.3M \\ 
6, 6, 1 & \best{41.954 / 0.884 / 15.127 / 1.082} & 473G & 17.4M \\\hline
\textbf{6, 4, 1} & \secondBest{41.678 / 0.899 / 15.201 / 1.091} & 454G & 17.0M \\ %
\bottomrule[0.15em]
\end{tabular}
}}
\vspace*{-1mm}
\end{table*}


==> tables/005_demo.tex <==
%
\begin{table}[t]
\begin{center}
\caption{\small \underline{\textbf{HSI restoration results with single degradation}}. Following PromptIR~\cite{PromptIR}, we train and evaluate the proposed method in all-in-one image restoration task, our method outperforms PromptIR across all the benchmark datasets.}
\label{table:all_in_one_restoration_results}
\vspace{-3mm}
\setlength{\tabcolsep}{1.9pt}
\scalebox{0.63}{
\begin{tabular}{l | c | c | c c c | c }
\toprule[0.15em]
%\rowcolor{color3} 
   & \textbf{Dehazing} & \textbf{Derain} & \multicolumn{3}{c|}{\textbf{Denoise} on BSD68} & \textbf{Average} \\

\textbf{Method} & on SOTS & on Rain100L & $\sigma=15$ & $\sigma=25$ & $\sigma=50$ &  \\
\midrule[0.1em]
BRDNet~\cite{BRDNet} & 23.23/0.895 & 27.42/0.895 & 32.26/0.898 & 29.74/0.836 & 26.34/0.836 & 27.80/0.843  \\
LPNet~\cite{LPNet}   & 20.84/0.828 & 24.88/0.784 & 26.47/0.778 & 24.77/0.748 & 21.26/0.552 & 23.64/0.738 \\
FDGAN~\cite{FDGAN}   & 24.71/0.924 & 29.89/0.933 & 30.25/0.910 & 28.81/0.868 & 26.43/0.776 & 28.02/0.883 \\
MPRNet~\cite{MPRNet} & 25.28/0.954 & 33.57/0.954 & 33.54/0.927 & 30.89/0.880 & 27.56/0.779 & 30.17/0.899 \\
DL~\cite{DL} & 26.92/0.391 & 32.62/0.931 & 33.05/0.914 & 30.41/0.861 & 26.90/0.740 & 29.98/0.875 \\
AirNet~\cite{AirNet} & 27.94/0.962 & 34.90/0.967 & 33.92/0.933 & 31.26/0.888 & 28.00/0.797  & 31.20/0.910 \\
\midrule[0.1em]
PromptIR~\cite{PromptIR} & \underline{30.58}/\underline{0.974} & \underline{36.37}/\underline{0.972} & \underline{33.98}/\underline{0.933} & \underline{31.31}/\underline{0.888} & \underline{28.06}/\underline{0.799} & \underline{32.06}/\underline{0.913} \\
\textbf{Ours} & \textbf{31.63}/\textbf{0.980} & \textbf{37.58}/\textbf{0.979} & \textbf{34.01}/\textbf{0.933} & \textbf{31.39}/\textbf{0.890} & \textbf{28.18}/\textbf{0.802} & \textbf{32.56}/\textbf{0.916} \\
\bottomrule[0.15em]
\end{tabular}
}
\end{center}
\vspace{-4mm}
\end{table}
%
